Unsupervised Learning of Compositional Energy Concepts

Humans are able to rapidly understand scenes by utilizing concepts extracted from prior experience. Such concepts are diverse, and include global scene descriptors, such as the weather or lighting, as well as local scene descriptors, such as the color or size of a particular object. So far, unsupervised discovery of concepts has focused on either modeling the global scene-level or the local object-level factors of variation, but not both. In this work, we propose COMET, which discovers and represents concepts as separate energy functions, enabling us to represent both global concepts as well as objects under a unified framework. COMET discovers energy functions through recomposing the input image, which we find captures independent factors without additional supervision. Sample generation in COMET is formulated as an optimization process on underlying energy functions, enabling us to generate images with permuted and composed concepts. Finally, discovered visual concepts in COMET generalize well, enabling us to compose concepts between separate modalities of images as well as with other concepts discovered by a separate instance of COMET trained on a different dataset. Code and data available at https://energy-based-model.github.io/comet/.

==> figText/celebahq_clevr_decomp.tex <==
\begin{figure}
    \includegraphics[width=\linewidth]{fig/celebahq_clevr_3.pdf}
    \caption{\small Left: Illustration of the decomposition of CelebA-HQ images into separate energy functions. Each displayed generation corresponds to optimizing an individual energy function. Energy functions capture the factors hair color, background lighting, facial expression and skin color in a CelebA-HQ image. Right: Illustration of the decomposition of  CLEVR images into separate energy functions. Each displayed generation show an image when optimizing over a set of energy functions of increasing number. Energy functions capture objects, floor, and lighting. } 
    \label{fig:celebahq_clevr_decomp}
    \vspace{-10pt}
\end{figure}

==> figText/smoketest.tex <==
\begin{wrapfigure}{l}{0.5\textwidth}
\vspace{-6mm} 
\includegraphics[width=\linewidth]{fig/blank.png}
\vspace{-15pt}
\caption{\small Illustration of teaser figure.}
\vspace{5pt}
\label{fig:smoketest}

\end{wrapfigure}

==> tbl/disentangle_tbl.tex <==
\begin{figure}
\begin{minipage}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=1.0\linewidth]{fig/clevr_global_decomp_v4.pdf}
    % \vspace{-10pt}
    \caption{\small \textbf{CLEVR Decomposition.} Generations on CLEVR when optimizing over increasing number of energy functions.} 
    \label{fig:celebahq_clevr_decomp}
 \end{minipage}\hfill
\begin{minipage}[b]{0.65\textwidth}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccc}
 \toprule
 Model & Dim ($D$) & $\beta$ & Decoder Dist. & BetaVAE & MIG & MCC \\
 \midrule
 COMET & $64$ & -- & -- & $99.24$ & $21.48$ & $77.27$ \\
 $\beta$-VAE & $64$ & $4$ & Gaussian & $79.28$ & $15.15$ & $68.06$ \\
 \midrule
 $\beta$-VAE & $32$ & $4$ & Gaussian & $92.20$ & $13.39$ & $64.03$ \\
 $\beta$-VAE & $256$ & $4$ & Gaussian & $76.96$ & $11.60$ & $64.98$ \\
 \midrule
 $\beta$-VAE & $64$ & $16$ & Gaussian & $76.50$ & $12.94$ & $59.72$ \\
  $\beta$-VAE & $64$ & $1$ & Gaussian & $88.92$ & $10.40$ & $66.02$ \\
 \midrule
 $\beta$-VAE & $64$ & $4$ & Bernoulli & $86.36$ & $12.04$ & $65.36$ \\
 \bottomrule
 \end{tabular}
 }
  \captionof{table}{\textbf{Disentanglement Evaluation.} Quantitative evaluation on the Falcor3D dataset. \model enables better disentanglement across 3 common disentanglement metrics across different runs and seeds for training $\beta$-VAE.}
 \label{table:disentangle_quant}
\end{minipage}
\vspace{-10pt}
\end{figure}


==> text/broader_impacts.tex <==
\section*{Broader Impact}
Our work is a step towards the broad goal of building a system with  physical understanding of the scenes around it. A system with a broad physical understanding of its surrounding environment has many potential impacts in industrial domains such as enabling household robots that can help the elderly age in place by helping with household chores and monitoring medical treatment. On the other hand, errors in our scene understanding system, such as classifying an unstable multi-object structure as a single object, could be costly if the model were actually deployed. We do not foresee our model, as a preliminary research effort, to have any significant societal impact toward any particular group.

==> text/checklist.tex <==
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See \sect{sect:conclusion}} 
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See \sect{sect:conclusion}} 
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{See \sect{sect:complexity}}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{See \sect{sect:complexity}}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{We provide them in the supplement. Code will be provided upon paper acceptance.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{We provide them in the supplement.} 
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{We provide them in the supplement.} 
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

